DROID-SLAM in the Wild

We present a robust, real-time RGB SLAM system that handles dynamic environments by leveraging differentiable Uncertainty-aware Bundle Adjustment. Traditional SLAM methods typically assume static scenes, leading to tracking failures in the presence of motion. Recent dynamic SLAM approaches attempt to address this challenge using predefined dynamic priors or uncertainty-aware mapping, but they remain limited when confronted with unknown dynamic objects or highly cluttered scenes where geometric mapping becomes unreliable. In contrast, our method estimates per-pixel uncertainty by exploiting multi-view visual feature inconsistency, enabling robust tracking and reconstruction even in real-world environments. The proposed system achieves state-of-the-art camera poses and scene geometry in cluttered dynamic scenarios while running in real time at around 10 FPS. Code and datasets are available at https://github.com/MoyangLi00/DROID-W.git.

==> tab/epic_kitchen.tex <==
\begin{table*}[t]
\centering
\scriptsize
{
\begin{tabular}{lrrrrrrr}
\toprule

Method & \texttt{200-5000} & \texttt{20000-23000} & \texttt{23000-26000} & \texttt{26000-29000} & \texttt{29000-32000} & \texttt{32000-35000} & Avg.\\
\midrule

DROID-SLAM~\cite{teed2021droid} & 1.033 & - & - & - & - & 1.011 & - \\

WildGS-SLAM~\cite{zheng2025wildgs} & 1.507 & \textbf{0.515} & 0.708 & 1.169 & 1.044 & 1.311 & 1.042 \\

{\project{}} & \textbf{1.017} & 0.538 & \textbf{0.678} & \textbf{1.074} & \textbf{0.917} & \textbf{0.956} & \textbf{0.863} \\

\bottomrule
\end{tabular}
}
\caption{\textbf{Tracking Performance on EPIC-KITCHENS Dataset} (ATE RMSE $\downarrow$). This sequence is too long, so we divide it into several slices for every 3000 frames on \textbf{P02-20240209-184316} and evaluate per-slice performance.
} 
\label{tab:epic_tracking}
\end{table*}

==> tab/runtime_details.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{2pt}
{
    \begin{tabular}{lcccccc}
        \toprule
        \multirow{2}{*}{Modules} & 
        \multicolumn{2}{c}{Online} & 
        \multicolumn{2}{c}{Offline} &
        \multicolumn{2}{c}{Full System} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
         & Time (s) & FPS & Time (s) & FPS & Time (s) & FPS \\
        \midrule
        WildGS-SLAM~\cite{zheng2025wildgs} & 3.33 & 0.30 & 0.96 & 1.05 & 4.28 & 0.23 \\
        \project{} & 0.10 & 9.89 & 0.02 & 50.80 & 0.12 & 8.28 \\
        \bottomrule
    \end{tabular}
}
\caption{\textbf{Runtime analysis on WildGS-SLAM Mocap Datasets \cite{zheng2025wildgs}.} 
All runtime analysis is performed on an RTX~3090 GPU.}
\label{tab:runtime_wild}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{2pt}
{
    \begin{tabular}{lcccccc}
        \toprule
        \multirow{2}{*}{Modules} & 
        \multicolumn{2}{c}{Online} & 
        \multicolumn{2}{c}{Offline} &
        \multicolumn{2}{c}{Full System} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
         & Time (s) & FPS & Time (s) & FPS & Time (s) & FPS \\
        \midrule
        WildGS-SLAM~\cite{zheng2025wildgs} & 3.30 & 0.30 & 1.17 & 0.85 & 4.47 & 0.22 \\
        \project{} & 0.10 & 9.64 & 0.02 & 55.69 & 0.12 & 8.22 \\
        \bottomrule
    \end{tabular}
}
\caption{\textbf{Runtime analysis on Bonn RGB-D Dynamic Datasets \cite{palazzolo2019iros}.} 
All runtime analysis is performed on an RTX~3090 GPU.}
\label{tab:runtime_bonn}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{2pt}
{
    \begin{tabular}{lcccccc}
        \toprule
        \multirow{2}{*}{Modules} & 
        \multicolumn{2}{c}{Online} & 
        \multicolumn{2}{c}{Offline} &
        \multicolumn{2}{c}{Full System} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
         & Time (s) & FPS & Time (s) & FPS & Time (s) & FPS \\
        \midrule
        WildGS-SLAM~\cite{zheng2025wildgs} & 2.52 & 0.40 & 0.66 & 1.53 & 3.17 & 0.32 \\
        \project{} & 0.08 & 12.87 & 0.01 & 73.92 & 0.09 & 10.96 \\
        \bottomrule
    \end{tabular}
}
\caption{\textbf{Runtime analysis on TUM RGB-D Datasets \cite{sturm2012benchmark}.} 
All runtime analysis is performed on an RTX~3090 GPU.}
\label{tab:runtime_tum}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{2pt}
{
    \begin{tabular}{lcccccc}
        \toprule
        \multirow{2}{*}{Modules} & 
        \multicolumn{2}{c}{Online} & 
        \multicolumn{2}{c}{Offline} &
        \multicolumn{2}{c}{Full System} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
         & Time (s) & FPS & Time (s) & FPS & Time (s) & FPS \\
        \midrule
        WildGS-SLAM~\cite{zheng2025wildgs} & 3.08 & 0.32 & 2.50 & 0.40 & 5.57 & 0.18 \\
        \project{} & 0.10 & 9.98 & 0.02 & 61.80 & 0.12 & 8.59 \\
        \bottomrule
    \end{tabular}
}
\caption{\textbf{Runtime analysis on DyCheck \cite{gao2022dycheck} Datasets.} 
All runtime analysis is performed on an RTX~3090 GPU.}
\label{tab:runtime_dycheck}
\end{table}

==> tab/wildgs_tracking.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{4.5pt}
{
\begin{tabular}{lrrrrrrrrrr
!{\smash{\tikz[baseline]{\draw[densely dashed, gray!80, line width=0.8pt] (0pt,-2pt)--(0pt,8pt);}}}
r}
    \toprule
    Method & \texttt{ANYmal1} & \texttt{ANYmal2} & \texttt{Ball} & \texttt{Crowd} & \texttt{Person} & \texttt{Racket} & \texttt{Stones} & \texttt{Table1} & \texttt{Table2} & \texttt{Umbrella} & \textbf{Avg.} \\
    \midrule
    \multicolumn{12}{l}{\cellcolor[HTML]{EEEEEE}{\textit{RGB-D}}} \\ 
    Refusion~\cite{palazzolo2019iros} & 4.2 & 5.6 & 5.0 & 91.9 & 5.0 & 10.4 & 39.4 & 99.1 & 101.0 & 10.7 & 37.23\\
    DynaSLAM (N+G)~\cite{bescos2018dynaslam} & 1.6 & 0.5 & \rd 0.5 & 1.7 & \nd 0.5 & 0.8 & 2.1 & 1.2 & 34.8 & 34.7 & 7.84 \\
    NICE-SLAM~\cite{Zhu2022CVPR} & F & 123.6 & 21.1 & F & 150.2 & F & 134.4 & 138.4 & F & 23.8 & - \\
    DG-SLAM~\cite{xu2024dgslam} & 1.2 & 2.1 & 0.8 & 1.3 & 1.5 & 1.6 & 1.5 & 2.0 & 57.9 & 1.35 & 7.06 \\
    UP-SLAM~\cite{zheng2025upslam} & \rd 0.4 & 0.6 & 0.6 & 1.1 & 1.1 & 0.9 & \rd 1.0 & \nd 0.7 & \rd 3.6 & 0.8 & 1.08 \\
    
    \hdashline
    \noalign{\vskip 1pt}
    \multicolumn{12}{l}{\cellcolor[HTML]{EEEEEE}{\textit{RGB-only}}} \\ 
    DSO~\cite{Engel2017DSO} & 12.0 & 2.5 & 1.0 & 88.6 & 9.3 & 3.1 & 41.5 & 50.6 & 85.3 & 26.0 & 32.99 \\
    DROID-SLAM~\cite{teed2021droid} & 0.6 & 4.7 & 1.2 & 2.3 & \rd 0.6 & 1.5 & 3.4 & 48.0 & 95.6 & 3.8 & 16.17\\
    DynaSLAM (RGB)~\cite{bescos2018dynaslam} & 0.6 & \rd 0.5 & \rd 0.5 & \nd 0.5 & \fs 0.4 & \rd 0.6 & 1.7 & 1.8 & 42.1 & 1.2 & 5.19 \\
    MonoGS~\cite{matsuki2024monogs}& 8.8 & 51.6 & 7.4 & 70.3 & 55.6 & 67.6 & 39.9 & 24.9 & 118.4 & 35.3 & 47.99\\
    Splat-SLAM~\cite{sandstrom2024splat}& \rd 0.4 & \nd 0.4 & \nd 0.3 & \rd 0.7 & 0.8 & \rd 0.6 & 1.9 & 2.5 & 73.6 & 5.9 & 8.71\\
    MonST3R-SW~\cite{zhang2024monst3r} & 3.5 & 21.6 & 6.1 & 14.4 & 7.2 & 13.2 & 11.2 & 4.8 & 33.7 & 5.5 & 12.12 \\
    MegaSaM~\cite{li2024megasam} & 0.6 & 2.7 & 0.6 & 1.0 & 3.2 & 1.6 & 3.2 & 1.0 & 9.4 & \rd 0.6 & 2.40\\
    
    WildGS-SLAM~\cite{zheng2025wildgs} & \fs 0.2 & \fs 0.3 & \fs 0.2 & \fs 0.3 & 0.8 & \fs 0.4 & \fs 0.3 & \fs 0.6 & \fs 1.3 & \fs 0.2 & \fs 0.46\\

    TTT3R~\cite{chen2025ttt3r} & - & - & - & - & - & - & - & - & - & - & - \\

    {\project{}} & \nd 0.3 & \fs 0.3 & \fs 0.2 & \fs 0.3 & 0.7 & \nd 0.5 & \nd 0.4 & \rd 0.8 & \nd 3.8 & \nd 0.3 & \nd 0.74 \\
    
    \bottomrule
\end{tabular}
}

\caption{\textbf{Tracking Performance on our Wild-SLAM MoCap Dataset \cite{zheng2025wildgs}} (ATE RMSE $\downarrow$ [cm]). Best results are highlighted as \colorbox{colorFst}{\bf first}, \colorbox{colorSnd}{second}, and \colorbox{colorTrd}{third}. All baseline methods were run using their publicly available code. For DynaSLAM (RGB), initialization is time-consuming for certain sequences, and only keyframe poses are generated and evaluated. `F' denotes tracking failure.} 
\label{tab:mocap_tracking}
\end{table*}

% \begin{table*}[t]
% \centering
% % \footnotesize
% \scriptsize  
% \setlength{\tabcolsep}{4.5pt}
% {
% \begin{tabular}{lrrrrrrrrrrrr}
%     \toprule
%     Method & \texttt{ANYmal1} & \texttt{ANYmal2} & \texttt{Ball} & \texttt{Crowd} & \texttt{Person} & \texttt{Racket} & \texttt{Stones} & \texttt{Table1} & \texttt{Table2} & \texttt{Umbrella} & Avg. \\
%     \midrule
    
%     % {\project{} (Python)} & 0.8 & \fs 0.2 & \fs 0.2 & \fs 0.3 & 0.7 & \fs 0.4 & \rd 0.5 & \rd 0.8 & 4.8 & \fs 0.2 & \rd 0.86 \\
%     % {\project{} (CUDA)} & 1.0 & \fs 0.2 & \fs 0.2 & \fs 0.3 & 0.7 & \fs 0.4 & \fs 0.3 & \rd 0.8 & 5.1 & \nd 0.6 & 0.96 \\
    
%     {\project{} (MLP 2 iters)} & 1.1 & 0.2 & 0.2 & 0.3 & 0.7 & 0.5 & 0.3 & 0.8 & 7.2 & 0.6 & 1.19 \\

%     {\project{} (MLP 10 iters)} & 1.0 & 0.2 & 0.2 &  & 0.7 & 0.5 & 0.4 & 0.8 & 17.8 & 0.3 & - \\    

%     % {\project{} (w/o uncer clamp)} & 0.8 & 0.2 & 0.2 & 0.3 & 0.8 & 0.5 & 0.4 & 0.8 & 13.9 & 0.5 & 1.84 \\

%     {\project{} (DINOv3)} & 0.6 & 0.2 & 0.2 & 0.3 & 0.6 & 0.5 & 0.4 & 1.0 & 12.3 & 0.6 & 1.67 \\

%     % {\project{} (w/ uncer clamp)} & 1.0 & 0.2 & 0.2 & 0.3 & 0.7 & 0.5 & 0.4 & 0.8 & 14.7 & 0.3 & 1.92 \\

%     % {\project{} (w/ consis $\beta_s=0.5, \beta_c=1.0$)} & 1.6 & 0.2 & 0.2 & 0.3 & 0.8 & 0.4 & 0.4 & 0.8 & 6.6 & 0.3 & 1.16 \\

%     % {\project{} (w/o consis $\beta_s=0.5, \beta_c=0.0$)} & 1.0 & 0.2 & 0.2 & 0.3 & 0.8 & 0.5 & 0.4 & 0.8 & 8.1 & 0.3 & 1.26 \\

%     {\project{} (w/o consis $\beta_s=0.25, \beta_c=0.0$)} & 0.6 & 0.2 & 0.2 & 0.3 & 0.8 & 0.5 & 0.4 & 0.8 & 10.6 & 0.6 & 1.49 \\

%     {\project{} (w/o consis $\beta_s=0.5, \beta_c=0.0$)} & 0.9 & 0.2 & 0.2 & 0.3 & 0.8 & 0.5 & 0.4 & 0.8 & 10.6 & 0.3 & 1.50 \\

%     {\project{} (w/ consis $\beta_s=0.5, \beta_c=1.0$)} & 0.9 & 0.2 & 0.2 & 0.3 & 0.8 & 0.5 & 0.4 & 0.8 & 8.0 & 0.4 & 1.24 \\

%     {\project{} ($L_{\text{new}}$ $\beta_s=0.0, \beta_c=0.0$)} & 0.3 & 0.2 & 0.2 & 0.3 & 0.7 & 0.5 & 0.4 & 0.8 & 6.0 & 0.6 & 1.00 \\

%     {\project{} ($L_{\text{new}}$ $\beta_s=0.5, \beta_c=0.0$)} & 1.4 & 0.2 & 0.2 & 0.3 & 0.8 & 0.5 & 0.4 & 0.8 & 6.2 & 0.3 & 1.10 \\

%     {\project{} ($L_{\text{new}}$ $\beta_s=0.1, \beta_c=0.0$)} & 0.5 & 0.3 & 0.2 & 0.3 & 0.7 & 0.5 & 0.4 & 0.8 & 7.7 & 0.5 & 1.17 \\

%     {\project{} ($L_{\text{new}}$ $\beta_s=0.1, \beta_c=0.0$), filter} & 0.6 & 0.3 & 0.2 & 0.3 & 0.7 & 0.4 & 0.4 & 0.7 & 6.9 & 0.3 & 1.07 \\

%     {\project{} ($L_{\text{new}}$ $\beta_s=0.1, \beta_c=0.0$), filter, *} & 0.4 & 0.3 & 0.2 & 0.3 & 0.7 & 0.5 & 0.4 & 0.8 & 7.0 & 0.4 & 1.09 \\

%     {\project{} ($L_{\text{new}}$ $\beta_s=0.5, \beta_c=0.0$), filter, *} & 1.0 & 0.2 & 0.2 & 0.3 & 0.8 & 0.4 & 0.4 & 0.8 & 5.7 & 0.4 & 1.01 \\
    
%     {\project{} ($L_{\text{new}}$ $\beta_s=0.1, \beta_c=0.0$), filter, * \#} & 0.3 & 0.3 & 0.2 & 0.3 & 0.6 & 0.5 & 0.4 & 0.7 & 5.9 & 0.4 & 0.96 \\
    
%     {\project{} ($L_{\text{new}}$ $\beta_s=0.5, \beta_c=0.0$), filter, * \#} & 1.0 & 0.3 & 0.2 & 0.3 & 0.7 & 0.5 & 0.3 & 0.7 & 8.9 & 0.5 & 1.33 \\

%     {\project{} ($L_{\text{new}}$ $\beta_s=0.5, \beta_c=0.0$), filter, * $\blacktriangleright$} & 0.3 & 0.3 & 0.4 & 0.3 & 0.8 & 0.5 & 0.4 & 0.8 & 2.6 & 0.5 & 0.68 \\

%     {\project{} ($L_{\text{new}}$ $\beta_s=0.0, \beta_c=0.0$), filter, * $\blacktriangleright$} & 0.2 & 0.3 & 0.2 & 0.3 & 0.7 & 0.4 & 0.4 & 0.8 & 2.8 & 0.6 & 0.66 \\

%     % {\project{} ($L_{\text{new}}$ $\beta_s=0.5, \beta_c=0.0$), filter, *} & - & - & - & - & - & - & - & - & - & - & - \\
    
%     \bottomrule
% \end{tabular}
% }
% 
% \caption{\textbf{Ablation Studies for Tracking Performance on Wild-SLAM MoCap \cite{zheng2025wildgs} Dataset} (ATE RMSE $\downarrow$ [cm]). Best results are highlighted as \colorbox{colorFst}{\bf first}, \colorbox{colorSnd}{second}, and \colorbox{colorTrd}{third}. All baseline methods were run using their publicly available code. For DynaSLAM (RGB), initialization is time-consuming for certain sequences, and only keyframe poses are generated and evaluated. `F' denotes tracking failure. \textcolor{red}{Here, for the computation of $L_\text{new}$, I set $sim<0.5?0.0:sim$ to improve separability between dynamic objects and static objects. * denotes constraints of $D_{\text{min}}=3$, \# denotes the use of mono-depth for dino feats reprojection. $\blacktriangleright$ represents the affine transformation and softplus activation}.}
% \label{tab:mocap_tracking_ablation}
% \end{table*}


